Higher-Order Relations Skew Link Prediction in Graphs

The problem of link prediction is of active interest. The main approach to solving the link prediction problem is based on heuristics such as Common Neighbors (CN) -- more number of common neighbors of a pair of nodes implies a higher chance of them getting linked. In this article, we investigate this problem in the presence of higher-order relations. Surprisingly, it is found that CN works very well, and even better in the presence of higher-order relations. However, as we prove in the current work, this is due to the CN-heuristic overestimating its prediction abilities in the presence of higher-order relations. This statement is proved by considering a theoretical model for higher-order relations and by showing that AUC scores of CN are higher than can be achieved from the model. Theoretical justification in simple cases is also provided. Further, we extend our observations to other similar link prediction algorithms such as Adamic Adar. Finally, these insights are used to propose an adjustment factor by taking into conscience that a random graph would only have a best AUC score of 0.5. This adjustment factor allows for a better estimation of generalization scores.

==> extras/__latexindent_temp.tex <==
@misc{turnbull2019latent,
    title={Latent Space Modelling of Hypergraph Data},
    author={Kathryn Turnbull and Simón Lunagómez and Christopher Nemeth and Edoardo Airoldi},
    year={2019},
    eprint={1909.00472},
    archivePrefix={arXiv},
    primaryClass={stat.ME}
}


@article{doi:10.1198/Hoff2002Latent,
author = {Peter D Hoff and Adrian E Raftery and Mark S Handcock},
title = {Latent Space Approaches to Social Network Analysis},
journal = {Journal of the American Statistical Association},
volume = {97},
number = {460},
pages = {1090-1098},
year  = {2002},
publisher = {Taylor & Francis},
doi = {10.1198/016214502388618906},

URL = { 
        https://doi.org/10.1198/016214502388618906
    
},
eprint = { 
        https://doi.org/10.1198/016214502388618906
    
}

}


==> extras/abstract.tex <==
Link Prediction -- predicting links between unlinked entities based on existing links -- is a well-known problem in network science, for which multiple solutions have been formulated in the literature.
Moreover, in any real-world network, relations usually occur originally as hyperedges, and are then induced as edges to form a graph/network.
Existence of such underlying hyperedges, along with their effect on link prediction, is ignored at large while predicting links.
% Neither is any explicit hyperedge-based topological information used for link prediction, owing to the seeming self-sufficiency of the induced graph itself.
    
In the present work, we elucidate a certain bias caused by such underlying hyperedges, to show that they in fact aid link prediction.
This is done by first generating random hypergraphs ``equivalent'' to existing, real-world ones, and then performing similar experiments on both.
% Post that, we move towards identifying topological features from underlying hyperedges and show that they further aid in predicting links in their respective induced counterparts.
Experiments are conducted on few real and corresponding simulated networks.

==> extras/exp.tex <==
\subsection{Real Data} 
\subsection{Simulated Data}

==> extras/figures/coacting_figure.tex <==
\begin{figure}[!t]
\begin{tabular}{cc}
    \includegraphics[scale=0.18]{images/co-actor-graph.png} & 
    \includegraphics[scale=0.18]{images/co-actor-hypergraph.png}\\
    (a) & (b)
\end{tabular}
\caption{Co-actors from the classic movie, \textit{Titanic}, where nodes represent actors. (a) How link prediction uses the co-acting relation (as ${6}\choose{2}$ = 15 induced pairwise relations/edges). (b) How the relation actually occurs (a single, 6-way relation or a 6-sized hyperedge).}
\label{fig:coacting}
\end{figure}

==> extras/preamble.tex <==
\pdfpagewidth=8.5in
\pdfpageheight=11in
% The file ijcai20.sty is NOT the same than previous years'
\usepackage{ijcai20}
\usepackage{amsmath, amssymb}
% \newtheorem{definition}{Def.}
\newcommand{\powerset}{\raisebox{.15\baselineskip}{\Large\ensuremath{\wp}}}

% Use the postscript times font!
\usepackage{times}
\usepackage{soul}
\usepackage{url}
\usepackage[hidelinks]{hyperref}
\usepackage[utf8]{inputenc}
\usepackage[small]{caption}
% \usepackage{bbold}
\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{algorithmic}
\urlstyle{same}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
% the following package is optional:
%\usepackage{latexsym} 

% See https://www.overleaf.com/learn/latex/theorems_and_proofs
% for a nice explanation of how to define new theorems, but keep
% in mind that the amsthm package is already included in this
% template and that you must *not* alter the styling.
\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}

% Following comment is from ijcai97-submit.tex:
% The preparation of these files was supported by Schlumberger Palo Alto
% Research, AT\&T Bell Laboratories, and Morgan Kaufmann Publishers.
% Shirley Jowell, of Morgan Kaufmann Publishers, and Peter F.
% Patel-Schneider, of AT\&T Bell Laboratories collaborated on their
% preparation.

% These instructions can be modified and used in other conferences as long
% as credit to the authors and supporting agencies is retained, this notice
% is not changed, and further modification or reuse is not restricted.
% Neither Shirley Jowell nor Peter F. Patel-Schneider can be listed as
% contacts for providing assistance without their prior permission.

% To use for other conferences, change references to files and the
% conference appropriate and use other authors, contacts, publishers, and
% organizations.
% Also change the deadline and address for returning papers and the length and
% page charge instructions.
% Put where the files are available in the appropriate places.

\newcommand{\NL}{N\!L}

\newcommand{\algrule}[1][.2pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}
\usepackage{arydshln}

==> extras/review_summary.tex <==
In this article we propose a novel insight into the working of  link prediction algorithms in presence of higher order relations. We have earlier submitted this article to IJCAI 2020.

The main reason for rejection is stated as - While the insight is interesting and novel, a way to use this insight was not convincing. In this version, we use the insight to propose a new evaluation method and provide extensive experiments where we evaluate existing link prediction heuristics.

The reviewers also misinterpreted the work stating that a new link prediction algorithm was proposed. However, this was not our aim. The exposition is substantially improved to better put forward this point. In particular figure 5 (current text) is added to better explain the reasoning behind the insight.

==> extras/sections/bkgd.tex <==
Given a set $S$, we denote by $|S|$, $\powerset(S)$, and $\powerset_k(S)$, its \textit{cardinality/size}, its \textit{power set}, and set of its \textit{$k$-sized subsets} respectively.
If $V$ is a set of \textit{nodes}/\textit{vertices}, a \textit{graph} is defined as $G := (V, E)$, where $E \subseteq \powerset_2(V)$ is the set of \textit{edges}.
Let $\mathbb{G}$ denote the set of all finite graphs.
For node $v \in V$, the set $\Gamma(v) := \{u\in V ~|~ \{u, v\} \in E\}$ is defined as its \textit{neighborhood}.
\textit{Density} of graph $G = (V, E)$ is defined as $\Delta(G) :=  \frac{2\cdot|E|}{|V|\cdot(|V| - 1)}$, \textit{i.e.}, the ratio of the number of actual edges to that of possible edges.

A \textit{$\rho$-split} of edges $E$ is defined as its binary partition $\Pi_{\rho}(E) := (E_{obs}, E_{unobs})$ into observed and unobserved edges respectively, in such a way that $|E_{obs}| = \rho \cdot |E|$ and $|E_{unobs}| = (1 - \rho) \cdot |E|$.
The \textit{link prediction problem} pertains to predicting unobserved links $E_{unobs}$ using information from observed ones, $E_{obs}$.
Finally, a set of non-links $\hat E$ is sampled from the set of non-links ($\hat E \subseteq \powerset_2(V) \setminus E$), so that a link prediction dataset comprising of observed links $E_{obs}$, unobserved links $E_{unobs}$, and non-links $\hat E$ could be prepared for a fair link prediction experiment.
% A \textit{$d$-hop non-link}~\cite{Lichtenwalter2010} is a pair $\{u, v\} \in \powerset(V) \setminus E$ such that $1 \lneq gd(u, v) \leq d$, where $gd$ denotes the geodesic distance between nodes $u$ and $v$. 
% Ideally, $d > 1$. Set of all $d$-hop non-links is denoted by $\NL^{(d)}(G)$.
A \textit{link predictor} $\mathcal{P}$ is a function that takes a link prediction dataset as input and returns a numeric score to each unobserved link and non-link corresponding to its probability of forming a link.

% \begin{table}[!htbp]
%     \caption{Link Prediction Algorithms used in the present work.}
%     \label{tab:lp_algorithms}
%     \centering
%     \input{tables/lp_algorithms.tex}
% \end{table}

A \textit{hypergraph} is defined as $H := (V, F)$, where $F \subseteq \powerset(V)$ is the set of \textit{hyperedges} over $V$.
The set of hyperedges incident to a given node $v \in V$ constitute its \textit{hyperneighbors} (or its \textit{hyperneighborhood}), and is denoted by $\tilde\Gamma(v) := \{e \in F~|~v \in e\}$.
Every hypergraph $H = (V, F)$ could be \textit{clique-expanded} into a graph $G = \eta(H) = (V, \eta(F))$, where $\eta(F) := \bigcup_{f \in F}\powerset_2(f)$.
We define the \textit{width} $\omega(H)$ of $H$ as $\max_{f \in F}|f|$.

==> extras/sections/conc.tex <==
Hyperedges are seldom talked about in the link prediction literature. We highlight their presence, their implications on networks in general, and its effect on link prediction. We set out to (1) elucidate the hidden data bias that hyperedge-derived networks possess, and (2) exploit information thereof explicitly to better predict links. It \textit{is} of concern that link prediction algorithms do not acknowledge the role of underlying hyperedges, and hence report incorrect performances (with the extent of incorrectness depending upon the hyperedge size distribution, their relative placement, etc.).
Ideally, be it structural or temporal, the main motive behind link prediction is to understand subtleties in a given network.
It does make use of structural topological properties to populate prediction scores, but scores ought be \textit{driven} by topology, not \textit{biased} by it.

In the foregoing sections, we have dealt with empirically elucidating the hyperedge bias that partially causes link prediction algorithms to perform. To do so, we compare results from two networks: real, and randomly-relocated.
We go a step further, and provide ways to extend our observations to \textit{aid} link prediction.

We conclude our work by saying that we found enough evidence to claim that there is, in fact a data bias that derived networks suffer from (or flourish on; depends on how it's viewed). And as the secondary goal of this work, information from the data bias could be explicitly used in the link-prediction pipeline to get decent uplift in performance.

% \section{Future Work}
% There are ample directions towards enhancing the current work:
% \begin{itemize}
%     \item From the link predictions' side, we are yet to explore a huge number of other techniques, \textit{viz.}, adjacency matrix factorization based, and those based on embedded-features.
%     \item Further, $BCI$-induction is not the final word for derived networks and numeric/fractional variants have immense potential for weighted link prediction.
%     \item We restricted ourselves to a large extent, esp. \textit{w.r.t.} dealing with only simple, undirected graphs, undirected hypergraphs, and structural link prediction. Directed graphs, hypergraphs, temporal link prediction is hugely studied in the literature and deserve bulk attention in terms of the foregoing analysis.
%     \item Generating random hypergraphs equivalent to real ones is a non-trivial problem, which has interested us during our analysis, and we were able to come up with a relocation procedure. This could be enhanced and interesting theoretical results could be established.
%     \item Finally, we would like to extend our arguments from the empirical to the theoretical paradigm, and would like to establish important such results. 
% \end{itemize}


==> extras/sections/exp.tex <==
\subsection{Datasets}
We pick real-world datasets from a recent work~\cite{benson}, which compiles several hypergraph networks for hyperlink (\textit{i.e.}, higher-order link) prediction (\textit{ref.} Table~\ref{tab:real-datasets}). During experimentation, all these datasets are to be converted into their $BCI$-induced versions and hence would be used as derived networks.

\begin{table}[!htbp]
    \caption{Description of real-world datasets used. $|V|$: number of nodes, $|F|$: number of hyperedges, $|E|$: \# $BCI(F)$.}
    \label{tab:real-datasets}
    \centering
    \input{tables/real-datasets.tex}
\end{table}
\vspace{-4mm}
We also use relocated counterparts of these networks (derived from Alg.~\ref{alg:relocated_hyg}) to get random derived networks for comparison. Let's denote a pair of real-relocated networks as $(G, G_{rel})$.

\subsection{Bias-exposing Experiments}
\label{sec:exp_results:bias}
For exposing data bias (\textit{ref.} Section~\ref{sec:lp_derived:databias}) while performing link prediction on derived datasets, we use pairs $(G, G_{rel})$ of real-world (\textit{ref.} Table~\ref{tab:real-datasets}) and relocated derived networks. For each real-world hypergraph $H$, we first induce a network $G$ as per Eq.~(\ref{eq:bci}). Then as per Section~\ref{sec:bkgd:lp}, we set $\rho = 0.8$ for an $80$-$20$ train-test graph $\rho$-split, and prepare the link prediction dataset, where $d$-hop non-links are sampled by setting $d = 2$. Then, each algorithm from Table~\ref{tab:lp_algorithms} is applied and average precision scores are reported in Table~\ref{tab:real_rel_scores}. The exact same steps are performed for relocated versions $G_{rel}$, and scores are populated against ``(rel)'' rows in Table~\ref{tab:real_rel_scores}. Entries where relocated versions are absolutely good (better than a threshold 0.1) are merely \textbf{bolded}. And cases where relocated versions perform better than real ones, corresponding entries are \textit{italicized} as well. Others are kept in the normal font.

% Figure~\ref{fig:real_rel_perc_inc_density} shows the percent increase in induced graph density when hypergraph is relocated.

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[scale=0.6]{images/real_rel_perc_inc_density.png}
%     \caption{\% Increase in Density when hypergraph is relocated.}
%     \label{fig:real_rel_perc_inc_density}
% \end{figure}

% Figure~\ref{fig:real_rel_scores_diff} shows the \% increase in \textit{\textbf{Average Precision}} when links are predicted on relocated hypergraphs.

\begin{table}[!htbp]
    \caption{Comparative analysis of average precision scores on $(G, G_{rel})$ pairs. }
    \label{tab:real_rel_scores}
    \centering
    \input{tables/real_rel_scores.tex}
\end{table}

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[scale=0.7]{images/real_rel_scores_diff.png}
%     \caption{\% Increase in $APr$ for LP on relocated hypergraphs. [??? TRANSPOSE THIS FIGURE BY DATASETS ON Y-AXIS AND ALGORITHMS AS LEGEND ???]}
%     \label{fig:real_rel_scores_diff}
% \end{figure}

% \subsection{Link Prediction through PHILiP}
% Here we consider only real-world networks, since our aim is to compare hypergraph-based features against existing algorithm-scores based ones. As explained in the concluding part of Section~\ref{sec:hyp_feats}, data matrices $\mathbf{X}^{alg}$ and $\mathbf{X}$ are computed for all real networks mentioned in Table~\ref{tab:real-datasets}. To compute $\mathbf{X}^{alg}$, the exact same parameters are used as in Section~\ref{sec:exp_results:bias}. Then we train classifiers that differentiate links from non-links (akin to~\cite{zaki}) and report evaluation results below. For classification, a $70$-$30$ train-test split is performed\footnote{This is a supervised learning (classifier) based train-test split and is not to be confused with $\rho$-split (\textit{ref.} Section~\ref{sec:bkgd:lp}) done to prepare a link prediction dataset.}.

% Table~\ref{tab:P@+_w_wo_hyg} shows $P@+$ scores (as defined in Eq.~(\ref{eq:p@k})) for classifiers for each $(\mathbf{X}^{alg}, \mathbf{X})$ pair. Entries where additional hypergraph features improve performance are \textbf{bolded}, with an upwards arrow $\uparrow$, and reduced performance is denoted by a downwards arrow $\downarrow$. There are cases where entries don't change \textit{w.r.t.} their $\mathbf{X}^{alg}$ counterparts. Such entries are suffixed with an up-down arrow $\updownarrow$. The last column ($*$-marked) in the table corresponds to our final conclusion based on each classifier's results. A $\uparrow$ denotes increase, $\downarrow$ denotes decrease, and $?$ means the results were ``inconclusive''.

% \begin{table}[!htbp]
%     \caption{$P@+$ scores for classifiers applied on $\mathbf{X}^{alg}$ (denoted by classifier name) and $\mathbf{X}$ (denoted by ``(hyg)'').}
%     \label{tab:P@+_w_wo_hyg}
%     \centering
%     \input{tables/P@+_w_wo_hyg.tex}
% \end{table}


% \begin{table}[!htbp]
%     \caption{$P@+$ scores for LP Algorithms w/o Hypergraph Features}
%     \label{tab:P@+_wo_hyg}
%     \centering
%     \input{tables/P@+_wo_hyg.tex}
% \end{table}

% \begin{figure*}[!htbp]
%     \centering
%     \includegraphics[scale=0.7]{images/P@+_wo_hyg.png}
%     \caption{$P@+$ scores for LP Algorithms w/o Hypergraph Features}
%     \label{fig:P@+_wo_hyg}
% \end{figure*}

% \begin{table}[!htbp]
%     \caption{$P@+$ scores for LP Algorithms with Hypergraph Features}
%     \label{tab:P@+_w_hyg}
%     \centering
%     \input{tables/P@+_w_hyg.tex}
% \end{table}

% \begin{figure*}[!htbp]
%     \centering
%     \includegraphics[scale=0.7]{images/P@+_w_hyg.png}
%     \caption{$P@+$ scores for LP Algorithms with Hypergraph Features}
%     \label{fig:P@+_w_hyg}
% \end{figure*}


==> extras/sections/hyp_feats.tex <==
As shown earlier (Section~\ref{sec:lp_derived}), a hypergraph-induced network has a certain bias, which affects link-prediction algorithms, be it favourably or otherwise. In other words, much of what the standard algorithms \textit{\textbf{capture}}, might only be the topological hypergraph-derived properties, and not the actual subtle factors which evolved the network to its current form. Although the latter claim is not too provable, we argue that more hypergraph features could be used to improve link prediction further. In other words, instead of implicitly (rather unknowingly) using a few features from the parent hyperedges, one could explicitly derive such features and more, and could expect a flow of information that improves link prediction further.

We list the additional features we think are important for link prediction in Table~\ref{tab:hyg_feats}. Most of these definitions use concepts explained in Section~\ref{sec:bkgd:hypergraphs}. To reiterate, all the features apply to an unordered pair $\{u, v\} \in \powerset_2(V)$. The reader is strongly referred to Sections~\ref{sec:bkgd:graphs} and~\ref{sec:bkgd:hypergraphs} to resolve symbolism. Here, $JC(A, B) := \frac{|A\cap B|}{|A \cup B|}$ represents the Jaccard Coefficient between two sets.

\begin{table}[!htbp]
    \caption{Parent Hyperedge Induced Features to enhance Link Prediction.}
    \label{tab:hyg_feats}
    \centering
    \begin{tabular}{rl}
        \toprule
        Feature & Formula\\
        \midrule
        $s_{max\omega}(u, v)$ & $\max(\{\omega(u), \omega(v)\})$ \\
        $s_{min\omega}(u, v)$ & $\min(\{\omega(u), \omega(v)\})$\\
        $s_{max\tilde\delta}(u, v)$ & $\max(\{\tilde\delta(u), \tilde\delta(v)\})$ \\
        $s_{min\tilde\delta}(u, v)$ & $\min(\{\tilde\delta(u), \tilde\delta(v)\})$ \\
        $s_{nc\tilde\Gamma}(u, v)$ & $\tilde\Gamma_{nc}(u, v) := \tilde\Gamma(u) ~\triangle~ \tilde\Gamma(v)$ \\
        $s_{o\tilde\Gamma}(u, v)$ & $|\{(e, f) \in \tilde\Gamma(u) \times \tilde\Gamma(v): e \cap f \neq \emptyset\}|$\\
        $s_{max\tilde\Gamma o}(u, v)$ & $\max_{(e, f) ~\in~ \tilde\Gamma(u) \times \tilde\Gamma(v)} JC(e, f)$ \\
        $s_{min\tilde\Gamma o}(u, v)$ & $\min_{(e, f) ~\in~ \tilde\Gamma(u) \times \tilde\Gamma(v)} JC(e, f)$ \\
        $s_{avg\tilde\Gamma o}(u, v)$ & $\displaystyle \frac{1}{\tilde\delta(u)\cdot\tilde\delta(v)}\sum_{(e, f) ~\in~ \tilde\Gamma(u) \times \tilde\Gamma(v)} JC(e, f)$\\
        \bottomrule
    \end{tabular}
\end{table}

There are many more hypergraph-specific features that could be used to predict links, but these basic ones serve as decent starting points and are sufficient to show a change in performance in link prediction. Here follows an explanation of each feature used:
\begin{enumerate}
    \item $s_{max\omega}(u, v)$: Maximum size of incident hyperedge
    \item $s_{min\omega}(u, v)$: Minimum size of incident hyperedge
    \item $s_{max\tilde\delta}(u, v)$: Maximum hyperdegree
    \item $s_{min\tilde\delta}(u, v)$: Minimum hyperdegree
    \item $s_{nc\tilde\Gamma}(u, v)$: Number of non-collaborations
    \item $s_{o\tilde\Gamma}(u, v)$: Number of overlaps
    \item $s_{max\tilde\Gamma o}(u, v)$: Maximum overlap
    \item $s_{min\tilde\Gamma o}(u, v)$: Minimum overlap
    \item $s_{avg\tilde\Gamma o}(u, v)$: Average overlap
\end{enumerate}


For each pair $p \in \powerset_2(V)$, two sets of features -- hypergraph-oriented topological features $\mathbf{x}^{hyg}(p) \in \mathbb{R}^{9}$, and algorithmic scores $\mathbf{x}^{alg}(p) \in \mathbb{R}^{8}$ are calculated, which concatenate to a single feature vector $\mathbf{x}(p) \in \mathbb{R}^{17}$. The corresponding data matrices could be represented by $\mathbf{X}^{hyg}$, $\mathbf{X}^{alg}$, and $\mathbf{X}$. To study the contribution of hypergraph-based features, we compare $P@+$ scores while (1) considering only $\mathbf{X}^{alg}$, and (2) considering both $\mathbf{X}^{alg}$ and $\mathbf{X}^{hyg}$ (\textit{i.e.},  $\mathbf{X}$).

==> extras/sections/hyperedge_nw.tex <==
It has been observed that, more often than not, link prediction is performed on networks that are \emph{possibly biased}, owing to their underlying hypergraph structure. Let's call such networks \textbf{\textit{hypergraph-derived}}\footnote{Throughout our discussion, ``derived'', ``hypergraph-derived'', ``hyperedge-derived'', ``induced'', ``hypergraph-induced'', and ``hyperedge-induced'' networks mean the same.} (or \textbf{\textit{derived}} for short), as opposed to networks that occur originally as graphs, called \textbf{\textit{native}} networks. For more clarity, let's make an attempt to formally define these terms.

\begin{definition}[\textbf{\textit{Native Graph / Network}}] Loosely speaking, we term a graph $G = (V, E)$ \textbf{native}\footnote{We choose ``native'' as an adjective for such graphs since they natively occur as graphs and not as higher-order hypergraphs.} and hence say $G \in \mathbb{G}_{nat}$ if the (binary) relation defined by $E$ occurs naturally and does not instead get inferred/induced from higher-order underlying relations.
\end{definition}

Some examples of native networks are ``friendship'', ``road-connectivity'', ``food-chain'', etc., since relations in them are naturally binary. A similar real-world definition of derived networks would be:
\begin{definition}[\textbf{\textit{Derived Graph / Network}}]
A graph that is not native is derived. In other words, \(G = (V, E)\) is \textbf{derived} -- \textit{i.e.}, $G \in \mathbb{G}_{der}$ -- if the relation defined by \(E\) does not occur naturally and was instead inferred/induced from a higher-order relation.
\end{definition}

Some examples of higher-order relations are: ``author-groups coauthoring a paper'', ``co-occurring word-groups'', ``drug-groups which should not be co-taken'', \textit{etc.}

\begin{definition}[Trivial/Non-trivial Hypergraph]
Hypergraphs with width at most 2 are called \textbf{trivial}, and those with width greater than 2 are called \textbf{non-trivial}. 
\end{definition}
% Some examples of such networks are listed in Table~\ref{tab:ex_derived_nw}.
% \begin{table*}[htb]
%   \caption{Some examples of derived networks.}
%   \label{tab:ex_derived_nw}
%   \input{tables/ex_derived_nw.tex}
% \end{table*}

\begin{lemma}
    \begin{equation}
        \mathbb{G} = \mathbb{G}_{nat} \cup \mathbb{G}_{der} \text{ and } \mathbb{G}_{nat} \cap \mathbb{G}_{der} = \emptyset.
    \end{equation}
\end{lemma}

\begin{lemma}
\label{lem:derived_graph_H}
For a given hypergraph $H \in \mathbb{H}$, we have:
\begin{equation}
     \eta(H) \in \mathbb{G}_{der} \iff \omega(H) \gneq 2.
\end{equation}
\end{lemma}

\begin{lemma}
\label{lem:derived_graph_G}
For a given graph $G \in \mathbb{G}$, we have:
\begin{equation}
     G \in \mathbb{G}_{der} \implies \exists ~H \in \mathbb{H} \text{ s.t. } \omega(H) \gneq 2 \text{ and } \eta(G) = H.
\end{equation}
\end{lemma}

\begin{lemma}
Converse of Lemma~\ref{lem:derived_graph_G} is not true. That is,
\begin{equation}
    \exists~G \notin \mathbb{G}_{der}, \exists~H \in \mathbb{H} \text{ s.t. } \omega(H) \gneq 2 \text{ and } \eta(G) = H.
\end{equation}
\end{lemma}

\subsection{Random Graphs}
\subsubsection{Random Native Network} $G(n, p) \in \mathbb{G}_{nat}$, a usual Erdos-Renyi random graph.

Suppose $CC$ is a random variable representing the clustering coefficient of $G$.

\begin{align}
    \mathbb{E}[CC] &= \frac{\mathbb{E}[\text{\# closed triangles}]}{\mathbb{E}[\text{\# connected triangles}]}\\
    &= \frac{3p^3}{3p^2(1-p) + 3p^3} = p
\end{align}

Also, let $CN$ denote the number of common neighbors between pairs of nodes in a random graph.
And since for any pair of nodes, $\{u, v\} \in \powerset_2(V)$, there are $n-2$ possible common neighbors $w \in V \setminus \{u, v\}$, each with probability $p^2$ of being a common neighbor, we have:

\begin{align}
    CN \sim Bin(n-2,~ p^2).
\end{align}
\begin{align}
    \implies \mathbb{E}[CN] &= (n-2)\cdot p^2.
\end{align}
\begin{align}
    Pr(\mathbf{1}_E=0) = 1-p
\end{align}
Also, $CN$ and $\mathbf{1}_E$ are independent, so:
\begin{align}
    \mathbb{E}[CN~|~\mathbf{1}_E=0] = \mathbb{E}[CN~|~\mathbf{1}_E=1] = \mathbb{E}[CN]
\end{align}

\subsubsection{Random Derived Network} $G(n, q, \alpha) \in \mathbb{G}_{der}$, clique-expansion $\eta(H)$ of a random hypergraph $H(n, q, \alpha)$.



==> extras/sections/intro.tex <==
Predicting links in networks is a well-known problem in network science, with applications ranging from recommending social connections, to mining unobserved protein interactions.
Ever since the almost seminal paper by Liben-Nowell, et al.~\cite{Liben-Nowell2003}, the area has seen constant research advancement, which recent review works~\cite{Martinez2016,Lu2010,Wang2015}, would testify. 

The problem basically refers to predicting new/missing links in a network.
For instance, given a \textit{co-authorship network} (a network of author-nodes wherein two of them get linked by an edge if and only if they co-author at least one publication), it is of interest to predict pairs of currently non-collaborating authors who are highly likely to collaborate in the future.
Similar is the case of a \textit{protein-protein interaction} (PPI) network (one where a pair of protein-nodes form an edge if and only if an \textit{in vitro/vivo} interaction between them is known to be observed), where the aim is to rank protein pairs in order of their interaction probability, which further helps prioritize \textit{in vitro} experiments. 

The two most popular types of link prediction problems are \textit{temporal} and \textit{structural}, which differ in their very intent.
While the former is used to study network evolution (of, say, a co-authorship network), the latter tries to predict hidden/missing links from a given (say, a PPI) network.
Irrespective of the problem type, the enormous link prediction literature provides many common similarity measures that get widely used in predicting links, either as individual scores~\cite{Liben-Nowell2003}, or as features to learn link predicting classifiers~\cite{AlHasan2006}.

This brings us to the crux of our work, \textit{viz.}, link prediction and \textit{hyperedges}, which, broadly defined, are structures that capture simultaneous interactions between multiple entities (as opposed to edges, which capture only pairwise interactions).
In the case of authors interacting to write papers for instance, a group of all authors who collaborate simultaneously on at least one paper qualify to form a hyperedge.
Another example of a hyperedge would be a group of proteins known to interact simultaneously.
In the literature, hyperedges have  seldom been discussed in the context of link prediction.
Nevertheless, our aim is to discuss the \textit{role} they play while links are predicted using well-known similarity measures.
\input{figures/coacting_figure.tex}

A typical network involves \textit{multi-way interaction of multiple entities at once} (except those that are by nature pairwise; e.g., \textit{friendship}).
Nevertheless, a link prediction pipeline inherently ignores the multi-way interactions and works with \textit{induced edges} instead.
Let us use a different example to understand this. 
Take a \textit{co-acting network} for instance, in which two actor-nodes form an edge if and only if they have both acted in the same movie at least once.
A toy network of this sort has been visualized in Fig.~\ref{fig:coacting}, where Fig.~\ref{fig:coacting}(b) refers to an originally occurring multi-way relation (hyperdge) between actors from a movie.
However, as a pre-processing step, any link prediction pipeline induces interacting pairs out of the hyperedge (the ones shown in Fig.~\ref{fig:coacting}(a)).
These pairs are then used to form link prediction models, and more links are predicted through them.

While the correctness of inducing links from a hyperedge and losses incurred therein could be subjects of another paper, we primarily focus on the \textbf{\textit{data bias}} that such a hyperedge brings to the link prediction table.
Most networks occur naturally as sets of hyperedges (called \textit{hypergraphs}), and are then induced into graph structures.
We focus on such underlying hyperedges and hypothesize that they \textit{\textbf{implicitly favor}} standard link-prediction algorithms.
Although since once induced into ${k}\choose{2}$ pairwise edges, a $k$-sized hyperedge loses its existence forever, any such bias seems impossible (owing to the mere nonexistence of the hyperedge in the network).
Hence we use the adjective ``implicit'' to describe the bias, in that the hyperedge passes bias to the induced graph structure implicitly.
One quick inference is as follows: \textit{portions of the network induced by larger hyperedges are denser than those by smaller ones}.
This is because on an average, larger hyperedges induce more edges, higher degrees, and higher clustering coefficients than smaller ones.

A loose yet interesting analogy is that of ``paper marbling''~\cite{wiki:paper_marbling} (painting on the surface of water).
Let us suppose an artist is allowed to use paint-brushes of different sizes to only pour droplets of black paint over the water surface, which eventually diffuse into surroundings to automatically form the painting.
The final painting would have dark, light, and medium patches of black color spatially diffused over the water surface, corresponding exactly to brush sizes.
In other words, smaller brushes would give lighter shades and larger ones, darker. Here, ``brush-size'' analogues to ``hyperedge-size'', dark shades to densely connected nodes, and lighter ones to sparse portions of the graph.

In the present work, we make attempts to elucidate data bias in link prediction due to the inherent role of underlying hyperedges.
We enumerate our contributions explicitly as follows:
\begin{enumerate}
    \item We present a novel empirical approach to \textbf{\textit{elucidate data-bias for link prediction}} caused by parent hyperedges.
\end{enumerate}

==> extras/sections/lp_derived.tex <==
In general, the basic goal of link prediction is to understand the evolution of networks. Typically, a link prediction algorithm aims to uncover the pragmatic factors that led to formation of links between real-world entities.
For example, two people having a large number of common friends are highly likely to be connected (or eventually get connected) as friends in a friendship network -- the well-known \textit{common-neighbor} argument. Hence, a typical link prediction algorithm is expected to model real-world subtleties in link evolution. 

But since derived networks inherit properties from their respective parent hypergraphs, the natural \textbf{\textit{subtleties}} that a given network evolved through, gets interfered with. In other words, we argue that for a derived network, most link prediction algorithms unknowingly focus on topological properties of the parent hypergraph and less on real-world subtleties. This is what we call the \textbf{\textit{data bias in link prediction}} due to derived networks.

Another way to state this argument is as follows: let's take two real-world networks $G_1$ and $G_2$ whose parent hypergraphs have similar topological properties (say similar \textit{number of nodes}, \textit{number of hyperedges}, \textit{hyperedge-size distributions}, and \textit{number of $BCI$-induced edges}). But both belong to different domains (say ``co-authorship'' and ``contact'' respectively). Since their respective $BCI$-induced counterparts too are similar in terms of information induced by parent hypergraphs, any link prediction algorithm would give similar results, which might be biased by the induced network's properties. In such a situation, it's difficult for any algorithm to ``measurably'' outperform the other, since the dataset itself was taken over by $BCI$-induced cliques.

\subsection{Empirical Elucidation of Data-bias}
\label{sec:lp_derived:databias}
Here, we describe the exact methodology by which we plan to expose data-bias in derived networks, providing in the process, justifications for the same.

Our argument is as follows: Link prediction is all about studying the structural or temporal evolution of connections in a real-world network. Let's suppose one attempts to predict links in a \textbf{\textit{random network}} -- say, an ER graph $G(n, p)$~\cite{erdos} -- or attempts to study its evolution~\cite{erdos_evolution} through a link prediction algorithm, it's \textbf{\textit{futile}} to say the least, since any link prediction algorithm would perform as good (or bad) as a random link-predictor\footnote{One that assigns random scores to test pairs $X_{test}$.}. The reason is simple: links in a random graph are formed \textit{at random}.

The same argument follows for derived networks too. That is, showing that certain link prediction algorithms \textit{\textbf{perform decently on random derived networks}} is enough to elucidate the said bias. In fact, we do exactly that: perform link prediction experiments on random derived networks. There's one road-block though: generating a random derived network equivalent to a given real-world one. This is necessary for a fair comparison between the two. We explicitly solve this problem as follows.

\subsection{Randomizing Derived Networks}
\label{sec:lp_derived:random}
To solve the foregoing problem of generating equivalent random derived networks, we need to be careful. While the field of random hypergraphs~\cite{ghoshal} is still evolving, we provide a \textit{\textbf{size-distribution preserving hypergraph relocation algorithm}} (Alg.~\ref{alg:relocated_hyg}), which explicitly replaces each hyperedge with a random hyperedge of the same size. As is clear from the process, it preserves the frequency distribution of hyperedge-sizes.

\begin{algorithm}[!htbp]
\caption{\textsc{RelocateHypergraph($H$)}}
\label{alg:relocated_hyg}
\begin{itemize}
     \item $H$: Given hypergraph $H = (V, F)$
 \end{itemize}
 \begin{algorithmic}[1]
 \algrule
 \STATE $F_{rel} \leftarrow \{\}$
 \FOR{$e \in F$}
 \STATE $e_{rel} \leftarrow$ \textsc{SampleWithoutReplacement}($V$, $|e|$)
 $F_{rel} \leftarrow F_{rel} \cup \{e_{rel}\}$
 \ENDFOR
 \STATE $H_{rel} \leftarrow (V, F_{rel})$
 \RETURN $H_{rel}$
 \end{algorithmic}
\end{algorithm}

Here, \textsc{SampleWithoutReplacement}($V$, $|e|$) uniformly samples a set of $|e|$ unique nodes from $V$.

For a given real-world derived network whose parent hypergraph is known to be $H$ (\textit{i.e.}, the derived network is $G = BCI(H)$), we first relocate all of its hyperedges to get an equivalent hypergraph $H_{rel}$. Inducing a network $G_{rel} = BCI(H_{rel})$ then gives us a random derived network which is equivalent to the real-world network $G$. In summary, we have with us two networks $G$ and $G_{rel}$, and we could perform link prediction on both to fairly establish data bias. More specifically, we say that data $G$ is biased for algorithm $A$ if $A$ performs well on $G_{rel}$ (which is a purely random network).



==> extras/sections/results.tex <==
Looking at Table~\ref{tab:real_rel_scores}, we note that predicting links on a randomly relocated network performs decently (if not better) in some cases. This very observation hints that randomly relocated hypergraphs provide sufficient conditions for some algorithms to perform well. This is because our main aim was to show that LP algorithms perform decently even on \textit{randomly relocated} derived networks, \textit{\textbf{which is not expected from a link prediction algorithm}}, since predicting links makes \textit{\textbf{little to no sense on random networks}}. While there are cases where the relocated network performs worse even in the absolute sense (\textit{e.g.}, for the c-h-s dataset), and reasons for the same should be analyzed, but in summary, one could say that \textbf{\textit{random derived networks give a fair chance}} for most well-known link prediction algorithms to perform. That said, we could also compare the results between algorithms, in that Preferential Attachment (PA)~\cite{barabasi,newman_pa} seems to have the least precision scores, probably owing to structural link prediction and not temporal. Further, SimRank (SR)~\cite{jeh} performs much better on real networks than relocated ones, which hints at its affinity to capture subtleties amidst noise due to parent-hypergraph-induced topological properties.

% Coming to Table~\ref{tab:P@+_w_wo_hyg}, which shows the effect of incorporating parent-hypergraph induced features in link prediction, we have the following observations. While for some classifiers (AdaBoost and NeuralNetworks), all datasets show increase in performance, for others (DecisionTree and RandomForest), there are irregularities. Nevertheless, as reported by the $*$-marked column, three out of six classifiers show an uplift, one (NaiveBayes) shows a consistent performance reduction, and two results remain inconclusive. Across datasets too, except c-p-s, all others have a single conclusive result: \textbf{\textit{additional hypergraph features aid link prediction performance}}. The actual aim of this experiment was to see whether using hypergraph features explicitly (instead of involuntarily) through a classifier helps the case for link prediction. And we could say that it does improve the performance of link prediction.

==> extras/sections/sota.tex <==
% \subsection{Link Prediction}
% \label{sec:sota:lp}
Link prediction has a huge literature, and covering it in whole is beyond the scope of the present work.
The reader is redirected to some excellent review works~\cite{Wang2014,Lu2010,Martinez2016}, which provide an intelligible coverage of the LP ecosystem.
Although the concept wasn't new to network scientists, and there have been vintage works on predicting new relations in networks~\cite{Katz1953}, the first formal work on LP could be credited to Liben-Nowell, \textit{et al.}~\cite{Liben-Nowell2003}.
They brought together multiple heuristics to solve the problem, heuristics both new as well as existing~\cite{Adamic2003}.
Ever since, many interesting directions to solve the problem were taken:
learning classifiers~\cite{AlHasan2006,Lu2010}, factorizing matrices~\cite{Menon2011,Miller2009} and tensors~\cite{Dunlavy2011,Acar2009}, building probabilistic models~\cite{Wang2007,Popescul2003,Sarukkai2000}, learning edge embeddings~\cite{Trouillon2016, Grover2016}, or directly learning a deep neural network~\cite{Li2014}.
None of these works acknowledge the role of hyperedges in link prediction.

% \subsection{Induced Networks}
% \label{sec:sota:lp_der_nw}
Networks induced from hypergraphs are the most frequently used datasets in the link prediction literature.
Even if popular applications are taken into account, they most of them deal with co-occurrence based relations, which are essentially induced from underlying hypergraphs.
All the link prediction works we mention here use derived networks of some kind or the other~\cite{AlHasan2006,Li2014,Liben-Nowell2003,Lu2010,Menon2011,Newman2004,Shibata2012,Wang2014}.
As we would show, performing link prediction on induced networks incurs an inherent bias in the process, which could be elucidated by perturbing the real nature of datasets used (we do this via relocating hyperedges in a real network).

% \begin{table}[htb]
% \caption{Datasets used in the literature.}
%     \label{tab:data_lit}
%     \centering
%     \input{tables/lp_and_derived_datasets.tex}
% \end{table}
% \subsection{Hypergraphs}
% \label{sec:sota:lp_hyg}
Though hyperedges and hypergraphs find place in many works on combinatorics~\cite{Berge1984,Bretto2013}, it's only recently that they have gained interest of computer and network scientists.
Another area where they are given importance is in biology, to model cellular and metabolite networks~\cite{Klamt2009,Zhang2016,Zhang2018}.
Though link prediction has been widely studied, almost all works (except a few~\cite{Li2013}) \textit{don't} consider the 
underlying hyperedge structure before the network gets converted to a graph.
Recently, there has been interest in the areas of \textit{hyperlink} (or simplex, or merely hyperedge) prediction as well, which acknowledge the fact that 
there's a loss of information when a hypergraph network is converted to a 
network~\cite{Xu2013,Benson2018,Sharma2014}, including deep learning to predict hyperlinks~\cite{Yadati2019}.

% \subsection{Bipartite and Heterogeneous Networks}
% While there has been a long going debate~\cite{hyg_vs_bip} about hypergraphs being equivalent to bipartite graphs (graphs with edges only in two sets of nodes), it is neither entirely true, nor false. In other words, mathematically, there \textit{is} a one-one correspondance between simple hypergraphs and simple bipartite networks (one could have all existing nodes in one set and dummy hyperedge nodes in another, and link an existing node to a hyperedge node with a bipartite edge if the latter is a hyperedge over the former). But from the perspective of link prediction, predicting bipartite links do not correspond to predicting hyperlinks (ref. Section~\ref{sec:sota:lp_hyg}).  Nevertheless, there has been considerable research on link prediction on bipartite networks~\cite{kunegis, benchettara} and a few on \textit{one-mode projections} (what we call as an \textit{induced} network) thereof into unipartite networks~\cite{allali, gao}. While link prediction on one-mode projections do have relevance to our work, since both are equivalent structures, we choose the hypergraphs terminology. 

% Another popular set of networks that should not be left unmentioned are heterogeneous networks.
% Again, akin to bipartite networks, in the context of link prediction, heterogeneous networks~\cite{sun, dong} (i.e., networks with multiple node and edge ``types'') too have equivalence with hypergraphs, and what we call induction, is referred to as ``homogenization''.

% Nevertheless, neither of them acknowledge the role of ``bipartiteness'' or ``heterogeneity'' in biasing the derived networks in favor of link prediction.


==> extras/table_AA_AUC.tex <==
\begin{tabular}{lcl}
\toprule
\textbf{Dataset} & \textbf{Original} & \textbf{Relocated} \\
\midrule
\textit{email-Enron}            &  $94.20$ &  $63.79\pm0.42$ \\
\textit{contact-high-school}   &  $93.69$ &  $55.06\pm0.39$ \\
\textit{contact-primary-school} &  $86.93$ &  $52.53\pm0.40$ \\
\textit{NDC-substances}         &  $99.08$ &  $98.94\pm0.001$\\
\textit{tags-math-sx}           &  $94.84$ &  $64.81\pm0.11$ \\ \bottomrule
\end{tabular}


==> extras/table_CN_AUC.tex <==
\begin{tabular}{lrr|cl|cl}
\toprule
&&&{Original} & {Relocated} & {Original} & {Relocated}\\
\textbf{Dataset $(H)$} & $|V|$ & $|F|$ & \textbf{$AUC(CN, \eta(H))$} & \textbf{$AUC(CN, \eta(H_{rel}))$} & \textbf{$AUC(AA, \eta(H))$} & \textbf{$AUC(AA, \eta(H_{rel}))$}\\
\midrule
\textit{email-Enron} & 148 & 1,436            &  $93.55$ &  $63.74\pm0.74$ &  $94.20$ &  $63.79\pm0.42$\\
\textit{contatct-high-school}& 327 & 7,818   &  $93.41$ &  $54.90\pm0.36$ &  $93.69$ &  $55.06\pm0.39$\\
\textit{contact-primary-school}& 242 & 12,704 &  $86.27$ &  $52.62\pm0.46$ &  $86.93$ &  $52.53\pm0.40$\\
\textit{NDC-substances}& 5,556 & 4,525         &  $98.98$ &  $98.87\pm0.003$ &  $99.08$ &  $98.94\pm0.001$\\
\textit{tags-math-sx}& 1,554 & 22,274           &  $94.28$ &  $64.59\pm0.16$ &  $94.84$ &  $64.81\pm0.11$\\
\bottomrule
\end{tabular}


==> extras/table_alt.tex <==
\hspace{-2cm}
\begin{tabular}{llllllllll}
\toprule
             &       &        &      &                PA &                AA &                CN &                JC &                RA &                SR \\
\midrule
\multirow{4}{*}{email-Enron} & \multirow{4}{*}{148} & \multirow{4}{*}{1,436} & H &           $82.46$ &           $94.22$ &           $93.12$ &           $95.36$ &           $96.41$ &           $88.82$ \\
             &       &        & H\_rel &  $67.60 \pm 0.31$ &  $69.28 \pm 0.37$ &  $69.19 \pm 0.39$ &  $69.55 \pm 0.42$ &  $69.45 \pm 0.36$ &  $68.29 \pm 0.27$ \\
             &       &        & AF &            $1.35$ &            $1.39$ &            $1.38$ &            $1.39$ &            $1.39$ &            $1.37$ \\
             &       &        & AAUC &           $61.08$ &           $67.78$ &           $67.48$ &           $68.60$ &           $69.36$ &           $64.83$ \\
\cline{1-10}
\cline{2-10}
\cline{3-10}
\multirow{4}{*}{contact-high-school} & \multirow{4}{*}{327} & \multirow{4}{*}{7,818} & H &           $67.05$ &           $93.69$ &           $93.55$ &           $93.20$ &           $93.81$ &           $92.50$ \\
             &       &        & H\_rel &  $56.72 \pm 0.17$ &  $54.86 \pm 0.19$ &  $54.82 \pm 0.19$ &  $53.15 \pm 0.21$ &  $54.86 \pm 0.20$ &  $56.72 \pm 0.12$ \\
             &       &        & AF &            $1.13$ &            $1.10$ &            $1.10$ &            $1.06$ &            $1.10$ &            $1.13$ \\
             &       &        & AAUC &           $59.34$ &           $85.17$ &           $85.05$ &           $87.92$ &           $85.28$ &           $81.86$ \\
\cline{1-10}
\cline{2-10}
\cline{3-10}
\multirow{4}{*}{contact-primary-school} & \multirow{4}{*}{242} & \multirow{4}{*}{12,704} & H &           $72.20$ &           $86.95$ &           $86.27$ &           $88.94$ &           $88.73$ &           $86.28$ \\
             &       &        & H\_rel &  $56.18 \pm 0.21$ &  $52.38 \pm 0.19$ &  $52.36 \pm 0.19$ &  $49.40 \pm 0.20$ &  $52.39 \pm 0.18$ &  $55.06 \pm 0.29$ \\
             &       &        & AF &            $1.12$ &            $1.05$ &            $1.05$ &            $0.99$ &            $1.05$ &            $1.10$ \\
             &       &        & AAUC &           $64.46$ &           $82.81$ &           $82.16$ &           $89.84$ &           $84.50$ &           $78.44$ \\
\cline{1-10}
\cline{2-10}
\cline{3-10}
\multirow{4}{*}{NDC-substances} & \multirow{4}{*}{5,556} & \multirow{4}{*}{4,525} & H &           $96.86$ &           $99.13$ &           $98.95$ &           $98.67$ &           $99.57$ &           $98.88$ \\
             &       &        & H\_rel &  $66.90 \pm 0.12$ &  $96.50 \pm 0.08$ &  $96.11 \pm 0.10$ &  $98.48 \pm 0.02$ &  $97.75 \pm 0.02$ &  $88.96 \pm 0.05$ \\
             &       &        & AF &            $1.34$ &            $1.93$ &            $1.92$ &            $1.97$ &            $1.96$ &            $1.78$ \\
             &       &        & AAUC &           $72.28$ &           $51.36$ &           $51.54$ &           $50.09$ &           $50.80$ &           $55.55$ \\
\cline{1-10}
\cline{2-10}
\cline{3-10}
\multirow{4}{*}{tags-math-sx} & \multirow{4}{*}{1,554} & \multirow{4}{*}{22,274} & H &           $90.48$ &           $94.88$ &           $94.31$ &           $89.43$ &           $96.04$ &           $94.78$ \\
             &       &        & H\_rel &  $56.09 \pm 0.06$ &  $64.81 \pm 0.06$ &  $64.69 \pm 0.06$ &  $65.23 \pm 0.07$ &  $64.85 \pm 0.06$ &  $60.10 \pm 0.04$ \\
             &       &        & AF &            $1.12$ &            $1.30$ &            $1.29$ &            $1.30$ &            $1.30$ &            $1.20$ \\
             &       &        & AAUC &           $80.79$ &           $72.98$ &           $73.11$ &           $68.79$ &           $73.88$ &           $78.98$ \\
\cline{1-10}
\cline{2-10}
\cline{3-10}
\multirow{4}{*}{NDC-substances} & \multirow{4}{*}{5,556} & \multirow{4}{*}{4,525} & H &           $96.86$ &           $99.13$ &           $98.95$ &           $98.67$ &           $99.57$ &           $98.88$ \\
             &       &        & H\_rel &  $66.90 \pm 0.12$ &  $96.50 \pm 0.08$ &  $96.11 \pm 0.10$ &  $98.48 \pm 0.02$ &  $97.75 \pm 0.02$ &  $88.96 \pm 0.05$ \\
             &       &        & AF &            $1.34$ &            $1.93$ &            $1.92$ &            $1.97$ &            $1.96$ &            $1.78$ \\
             &       &        & AAUC &           $72.28$ &           $51.36$ &           $51.54$ &           $50.09$ &           $50.80$ &           $55.55$ \\
\cline{1-10}
\cline{2-10}
\cline{3-10}
\multirow{4}{*}{tags-math-sx} & \multirow{4}{*}{1,554} & \multirow{4}{*}{22,274} & H &           $90.48$ &           $94.88$ &           $94.31$ &           $89.43$ &           $96.04$ &           $94.78$ \\
             &       &        & H\_rel &  $56.09 \pm 0.06$ &  $64.81 \pm 0.06$ &  $64.69 \pm 0.06$ &  $65.23 \pm 0.07$ &  $64.85 \pm 0.06$ &  $60.10 \pm 0.04$ \\
             &       &        & AF &            $1.12$ &            $1.30$ &            $1.29$ &            $1.30$ &            $1.30$ &            $1.20$ \\
             &       &        & AAUC &           $80.79$ &           $72.98$ &           $73.11$ &           $68.79$ &           $73.88$ &           $78.98$ \\
\bottomrule
\end{tabular}

==> extras/tables/P_+_w_wo_hyg.tex <==
\begin{tabular}{p{6mm}p{9mm}p{9mm}p{9mm}p{9mm}p{9mm}p{3mm}}
\toprule
{} & e-En & c-h-s & c-p-s & N-c & e-Eu & $*$ \\
\midrule
AB & 0.88 & 0.52 & 0.49 & 0.59 & 0.51 \\
(hyg) & \textbf{0.92} $\uparrow$ & \textbf{0.63} $\uparrow$ & \textbf{0.54} $\uparrow$ & \textbf{0.77} $\uparrow$ & \textbf{0.52} $\uparrow$ & $\uparrow$\\ \hdashline
DT & 0.87 & 0.52 & 0.54 & 0.65 & 0.51 \\
(hyg) & \textbf{0.90} $\uparrow$ & \textbf{0.53} $\uparrow$ & 0.50 $\downarrow$ & \textbf{0.72} $\uparrow$ & \textbf{0.56} $\uparrow$ & $\uparrow$\\ \hdashline
NB & 0.51 & 0.52 & 0.42 & 0.50 & 0.37 \\
(hyg) & 0.40 $\downarrow$ & 0.52 $\updownarrow$ & 0.42 $\updownarrow$ & 0.48 $\downarrow$ & 0.32 $\downarrow$ & $\downarrow$\\\hdashline
kNN & 0.85 & 0.52 & 0.50 & 0.50 & 0.48 \\
(hyg) & 0.85 $\updownarrow$ & 0.50 $\downarrow$ & 0.50 $\updownarrow$ & \textbf{0.53} $\uparrow$ & 0.32 $\downarrow$ & $?$\\\hdashline
NN & 0.86 & 0.52 & 0.35 & 0.44 & 0.33 \\
(hyg) & \textbf{0.94} $\uparrow$ & \textbf{0.89} $\uparrow$ & \textbf{0.49} $\uparrow$ & \textbf{0.77} $\uparrow$ & \textbf{0.36} $\uparrow$ & $\uparrow$\\\hdashline
RF & 0.89 & 0.50 & 0.50 & 0.62 & 0.50 \\
(hyg) & 0.88 $\downarrow$ & \textbf{0.54} $\uparrow$ & 0.48 $\downarrow$ & \textbf{0.72} $\uparrow$ & 0.48 $\downarrow$ & $?$\\
\bottomrule
\end{tabular}


==> extras/tables/lp_algorithms.tex <==
\begin{tabular}{lll}
\toprule
Algorithm & Class & Abbreviation \\
\midrule
Adamic Adar & \textit{Neighbor} & AA \\
Common Neighbor & \textit{Neighbor} & CN \\
Jaccard Coefficient & \textit{Neighbor} & JC \\
Preferential Attachment & \textit{Centrality} & PA \\
Katz-$\beta$ & \textit{Path} & K \\
Resource Allocation & \textit{Neighbor} & RA \\
Rooted PageRank & \textit{Eigenvector} & RPR \\
SimRank & \textit{Eigenvector} & SR \\
\bottomrule
\end{tabular}

==> extras/tables/lp_and_derived_datasets.tex <==
\begin{tabular}{p{1.5cm}p{5cm}}
\toprule
Reference & Datasets used \\
\midrule
\cite{liben} & Five co-authorship networks\\
\cite{zaki} & Two author-paper networks\\
\cite{}\\
\bottomrule
\end{tabular}

==> extras/tables/real-datasets.tex <==
\begin{tabular}{llrrr}
    \toprule
        Name & Abbr. & $|V|$ & $|F|$ & $|E|$\\
    \midrule
        email-Enron & e-En & 143 & 1,542 & 1,855\\
        contact-primary-school & c-p-s & 242 & 12,799 & 8,317 \\
        email-Eu & e-Eu & 998 & 25,791 & 29,927\\
        contact-high-school & c-h-s & 327 & 7,937 & 5,818 \\
        NDC-classes & N-c & 1,161 & 1,222 & 6,263\\
    \bottomrule
    \end{tabular}

==> extras/tables/real_rel_scores.tex <==
\begin{tabular}{p{8mm}p{5mm}p{5mm}p{5mm}p{5mm}p{5mm}p{5mm}p{5mm}p{5mm}}
\toprule
{} & K & PA & AA & SR & RPR & JC & CN & RA \\
\midrule
c-h-s & 0.46 & 0.05 & 0.47 & 0.37 & 0.44 & 0.41 & 0.45 & 0.48 \\
(rel) & 0.06 & 0.05 & 0.06 & 0.05 & 0.06 & 0.06 & 0.06 & 0.06 \\\hdashline
N-c & 0.32 & 0.16 & 0.41 & 0.47 & 0.26 & 0.25 & 0.32 & 0.67 \\
(rel) & \textbf{\textit{0.63}} & 0.02 & \textbf{\textit{0.70}} & \textit{0.20} & \textbf{\textit{0.55}} & \textbf{\textit{0.80}} & \textbf{\textit{0.64}} & \textbf{\textit{0.74}} \\\hdashline
e-Eu & 0.31 & 0.14 & 0.36 & 0.27 & 0.28 & 0.40 & 0.32 & 0.48 \\
(rel) & \textbf{0.14} & \textbf{0.12} & \textbf{0.15} & \textbf{0.13} & \textbf{0.13} & \textbf{0.17} & \textbf{0.15} & \textbf{0.15} \\\hdashline
e-En & 0.06 & 0.05 & 0.06 & 0.06 & 0.06 & 0.07 & 0.45 & 0.06 \\
(rel) & \textbf{\textit{0.28}} & \textbf{\textit{0.26}} & \textbf{\textit{0.29}} & \textbf{\textit{0.26}} & \textbf{\textit{0.27}} & \textbf{\textit{0.29}} & \textbf{0.28} & \textbf{\textit{0.28}} \\\hdashline
c-p-s & 0.38 & 0.21 & 0.40 & 0.30 & 0.37 & 0.50 & 0.38 & 0.46 \\
(rel) & \textbf{0.21} & \textit{\textbf{0.21}} & \textbf{0.21} & \textbf{0.21} & \textbf{0.21} & \textbf{0.21} & \textbf{0.21} & \textbf{0.21} \\
\bottomrule
\end{tabular}

==> extras/titular.tex <==
\title{The Role of Hypergraphs in Link Prediction}

% Single author syntax
\author{
    % Christian Bessiere
    % \affiliations
    % CNRS, University of Montpellier, France
    % \emails
    % pcchair@ijcai20.org
}

% Multiple author syntax (remove the single-author syntax above and the \iffalse ... \fi here)
% Check the ijcai20-multiauthor.tex file for detailed instructions
% \iffalse
% \author{
% First Author$^1$
% \and
% Second Author$^2$\and
% Third Author$^{2,3}$\And
% Fourth Author$^4$
% \affiliations
% $^1$First Affiliation\\
% $^2$Second Affiliation\\
% $^3$Third Affiliation\\
% $^4$Fourth Affiliation
% \emails
% \{first, second\}@example.com,
% third@other.example.com,
% fourth@example.com
% }
% \fi

